HexaConv

The effectiveness of Convolutional Neural Networks stems in large part from their ability to exploit the translation invariance that is inherent in many learning problems. Recently, it was shown that CNNs can exploit other invariances, such as rotation invariance, by using group convolutions instead of planar convolutions. However, for reasons of performance and ease of implementation, it has been necessary to limit the group convolution to transformations that can be applied to the filters without interpolation. Thus, for images with square pixels, only integer translations, rotations by multiples of 90 degrees, and reflections are admissible. Whereas the square tiling provides a 4-fold rotational symmetry, a hexagonal tiling of the plane has a 6-fold rotational symmetry. In this paper we show how one can efficiently implement planar convolution and group convolution over hexagonal lattices, by re-using existing highly optimized convolution routines. We find that, due to the reduced anisotropy of hexagonal filters, planar HexaConv provides better accuracy than planar convolution with square filters, given a fixed parameter budget. Furthermore, we find that the increased degree of symmetry of the hexagonal grid increases the effectiveness of group convolutions, by allowing for more parameter sharing. We show that our method significantly outperforms conventional CNNs on the AID aerial scene classification dataset, even outperforming ImageNet pre-trained models.

==> acknowledgement.tex <==
We would like to thank Taco Cohen for his ideas. Thanks to his guidance we were able to understand and implement this research in the limited amount of time.



==> discussion.tex <==
Our experiments show that P6 G-CNNs improve performance on datasets where these
symmetries clearly exist, and we show that these CNNs perform close to others
on datasets where symmetries are not obvious. We discuss several factors that
might still restrict the performance hexagonal convolutions, together with
possible improvements of hexagonal convolutions.

In rectangular convolution often a filter size of 3 is used, with 9 tiles in
total. The approximating hexagonal filter only has 7 tiles. Therefore,
hexagonal convolutions with filter size 3 will have the same computational
cost, but will train less effectively than rectangular convolutions.

Hexagonal G-convolutions require an image to be sampled during preprocessing.
This sampling can introduce errors, especially when sampling from low
resolution images. This could put hexagonal G-CNNs at a disadvantage compared
to rectangular G-CCNs.

Although in theory an implementation that splits the convolution into two
separate convolutions should improve performance, however, we found that the
overhead of performing two convolutions (that includes multiple tensor copies)
does in general not weight up against a axial convolution. Potential improvements
exists in not moving back to a general representation, i.e., implement the split
of the convolution not at the layer level, but at the network level. However, doing
so may limit the possible parameter settings.

In future work the hexagonal parity convolutions may be implemented. These
would save computation and remove the need for normalization corrections. Also,
the models have not been optimized for state of the art performance, and P6
convolutions still need to be validated at high performance.  Furthermore,
although implementation exists for P6M G-convolutions, P6M G-CNNs still need to
be tested. Often datasets exhibit mirroring symmetries, and P6M G-CNNs could
leverage mirroring invariance as an additional advantage.


==> lattices-and-symmetries.tex <==
%!TEX root = report.tex

Conventionally, images are sampled on a square lattice.
This lattice has various symmetries: we can shift each pixel in the horizontal or vertical direction by an integer amount, we can rotate the lattice by multiples of $90$ degrees, or we can mirror it.
In each case, the transformation maps each pixel onto another pixel in a distance-preserving manner, which is why we call them symmetries of the lattice.

\begin{minipage}[]{0.65\textwidth}
In order to increase the degree of weight sharing in a G-CNN, we would like to use a lattice that has a higher degree of symmetry.
As it turns out, the most symmetric lattice is the hexagonal lattice $\mathcal{H}$.
This lattice is generated by integer linear combinations of two basis vectors, $e_1$ and $e_2$, separated by a $60$ degree angle (see figure \ref{fig:hexgrid}). 
\\
\\
The hexagonal lattice has the following symmetries:
we can shift by an integer number of units in the $e_1$ or $e_2$ direction, rotate by a multiple of $60$ degrees, or mirror the whole lattice. In this paper we consider the groups $p6$ which includes the translational and rotational symmetries, and $p6m$, which additionally contains the mirror reflections.
\end{minipage}
\hfill
\begin{minipage}[]{0.24\textwidth}
\includegraphics[width=\textwidth]{figures/hexgrid.pdf}
\captionof{figure}{Hexagonal grid}
\label{fig:hexgrid}
\end{minipage}
\hspace{1cm}

\begin{figure}
\centering

\end{figure}



An element of $p6$ can be written as $g = (r, t)$ for $r$ a rotation by a multiple of $60$ degrees, and $t = u e_1 + v e_2$ a translation vector in the lattice.
Writing $r \cdot t$ for the action of a rotation on the lattice, the composition of two elements $g = (r, t)$ and $h = (r', t')$ is given by $gh = (r r', r \cdot t' + t)$ and the inverse by $g^{-1} = (r^{-1}, - r^{-1} \cdot t)$.



==> symmetrygroups.tex <==
%!TEX root = report.tex
Given a geometrical object $O$, a rigid transformation of $O$ transforms $O$ in
such a way that the distances between points in $O$ are unchanged. We call a
rigid transformation a symmetry of $O$ when after transforming $O$, $O$ looks
the same as before the transformation.  Formally, a \textit{symmetry} is a
function $f$ that maps $O$ onto itself such that the distance between $x$ and
$y$ in $O$ is the same as the distance between $f(x)$ and
$f(y)$~\citep{gowers2010princeton}, i.e., the object is invariant with respect
to the transformation.  For example, consider the rectangular sampling grid
\Ztwo, when we rotate \Ztwo by 90 degrees we obtain $\{(-v, u) \mid (u, v) \in
\Ztwo \} = \Ztwo$. Hence, the rotation by 90 degrees is a symmetry of \Ztwo.

We can examine collections of symmetries. Consider the set of all symmetries $S$ of an object. Let $g, h \in G$ then the composition $gh$ must also be in $S$, i.e., by first performing $h$ the object is left invariant,
then by performing $g$ the object is again left invariant, hence, $gh$ must
also be a symmetry of the object. Moreover, consider the transformation that undoes a transformation, this is called the inverse, and denoted by
$g^{-1}$ for a transformation $g$. If $g$ is an transformation that leaves the
object invariant, and $g^{-1}$ undoes this operation, then $g^{-1}$ must also
leave the object invariant, thus, $g^{-1} \in S$. As $g, g^{-1} \in S$, it
follows that $gg^{-1} \in S$, this is called the identity transformation and
does not change the object. The identity transformation is often denoted as
$e$. When a set satisfies these requirements it is called a \textit{symmetry
group}.

% As discussed, symmetry groups are the foundation of the work
% of~\cite{cohen2016group} on which we build on. More specifically, the symmetry
% group theory provides a unified approach to designing Group Equivariant
% Convolution operations (GConvs) that can be leveraged in Convolutional Neural
% Networks (CNNs). Next we will discuss the specific symmetry groups used in the
% present study.

\subsection{Symmetry Groups on Hexagonal Lattice} 
%% Story:
% Status
% Group theory
% Implication
Conventionally images are stored as sampled square grids, as pixels. This restriction is not a necessary fundamental property, but rather a result of sensor arrays in cameras. Alternatively, images can be stored using a grid composed of hexagons. 
In group theory, wallpaper groups are categorizing all possible symmetries with repetitive 2D patterns. Wallpaper groups are a natural description for images in group theory. The wallpaper groups with highest rotational symmetry are $p6$ and $p6m$, having rotations of 60 degrees. A hexagonal grid is an example of a structure that satisfies the properties of $p6$ and $p6m$. Analogously, a square grid satisfies the properties of $p4$ and $p4m$. Note that hexagonal grids also exemplify other wallpaper groups, but $p6(m)$ attains the highest rotational symmetry.
The groups $p6$ and $p6m$ have two additional rotational symmetries, compared to $p4$ and $p4m$. Thus, we can leverage group operations with high symmetry, by expressing images on hexagonal grids rather than square grids.


\subsubsection{The Group $p6$}
The group $p6$ is the group that contains all compositions of translations and rotations by 60 degrees, around any rotation center. A group operation $g$ can be composed as $g = (r, u, v)$, a combination of rotations ($r$) and translations ($u$ and $v$).
For example, two rotations followed by a single translation on both axes can be encoded with $(2, 1, 1)$. The actual element composition $gh$ for $g = (r, u, v)$ and $h = (r', u', v')$ depends on the choice of coordinate system, and will be discussed section~\ref{sec:hexcoord}. 
\TODO{We can actually discuss the composition in an abstract way if we refer to an abstract action of the rotation group C6 on the translation group.}

% it is computed by converting $(u', v')$ to the cube coordinate system using $t = (x, y, z) = (v', -(u'+v'), u')$, perform $r$
% rotations to obtain $t' = (x', y', z')$. Then convert $t'$ back to the axial coordinate system
% using $(u'', v'') = (z' + u, x'+ v)$ and add the translation components of $g$ to obtain the final translation. The rotation of the composed element is computed using $r'' = r + r' \mod 6$. Then $gh = (r'', u'', v'')$. 


% Although transformations can be defined in any coordinate system, the expressions in the cube coordinate system are straightforward. The computational overhead is negligible, since the results of the computation are cached.

% \footnote{Although $p6$ also has rotation centers of order two (three centers) and order three (two centers), these are not used in the present study.}

\subsubsection{The Group $p6m$}
The group $p6m$ is the group that contains all compositions of translations, rotations by 60 degrees and a mirror axis. The group is an extension of $p6$, and elements of $p6m$ can be encoded in a similar fashion as $p6$. In addition to the rotation and translation components, we express the current mirror state by a zero or one. For example, rotating twice, a mirror transformation and a translation of one for both axes, can be expressed as $(1, 2, 1, 1)$. Element compositions are computed in a similar fashion as the element compositions for $p6$. 


% The mirror transformation is computed after the rotation in the cube coordinate system, the mirror transformation is first computed in the cube coordinate system. Similarly,
% the mirror component is computed by summing both mirror components modulo two.

